Wave propagation in one-dimensional quasiperiodic media

This work is devoted to the resolution of the Helmholtz equation $-(\mu u')' - \rho \omega^2 u = f$ in a one-dimensional unbounded medium. We assume the coefficients of this equation to be local perturbations of quasiperiodic functions, namely the traces along a particular line of higher-dimensional periodic functions. Using the definition of quasiperiodicity, the problem is lifted onto a higher-dimensional problem with periodic coefficients. The periodicity of the augmented problem allows us to extend the ideas of the DtN-based method developed for the elliptic case. However, the associated mathematical and numerical analysis of the method are more delicate because the augmented PDE is degenerate, in the sense that the principal part of its operator is no longer elliptic. We also study the numerical resolution of this PDE, which relies on the resolution of Dirichlet cell problems as well as a constrained Riccati equation.

==> figures/figures.tex <==
% Pour corriger le bug du cercle
\makeatletter
\def\pgfplots@install@path@replacements{%
    \ifpgfplots@path@replace@ellipse
        \let\tikz@do@circle=\pgfplots@path@@tikz@do@circle
        \let\tikz@do@ellipse=\pgfplots@path@@tikz@do@circle
        \expandafter\def\expandafter\pgfinterruptpicture\expandafter{\pgfinterruptpicture
            \let\tikz@do@circle=\pgfplots@path@@tikz@do@circle@orig
            \let\tikz@do@ellipse=\pgfplots@path@@tikz@do@ellipse@orig
        }%
    \fi
}%
\let\pgfplots@path@@tikz@do@circle@orig=\tikz@do@circle
\let\pgfplots@path@@tikz@do@ellipse@orig=\tikz@do@ellipse

\let\pgfplots@path@@tikz@do@circle@oldandbroken=\pgfplots@path@@tikz@do@circle
\def\pgfplots@path@@tikz@do@circle#1{\pgfplots@path@@tikz@do@circle@oldandbroken{#1}{#1}}
\def\pgfplots@path@@tikz@do@ellipse#1#2{\pgfplots@path@@tikz@do@circle@oldandbroken{#1}{#2}}
\makeatother

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Style to select only points from #1 to #2 (inclusive)
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pour dessiner fibrages
\newcommand{\dessinerFibrage}[4]{
  % #1: number of iterations
  % #2: plot file for solid line
  % #3: plot file for dashed line
  % #4: boolean; should one show dashed line or not
  \begin{tikzpicture}
    \pgfmathsetmacro\nPtSolidMAX{3*#1}
    \pgfmathsetmacro\nPtDashedMAX{3*#1-2}
    \begin{axis}[
      width=0.95\textwidth, height=0.95\textwidth,
      xmin=0, xmax=1, ymin=0, ymax=1,
      xtick={0, 1}, ytick={0, 1},
      enlargelimits=false,
      axis equal,
      unbounded coords=jump]
      \ifthenelse{\boolean{afficherGraphes}}{
        \addplot[bleuDoux!75, line width=0.2mm, mark=*, mark options={scale=0.5}, select coords between index={0}{\nPtSolidMAX}] table[x={x}, y={y}] {#2};
        \ifthenelse{\boolean{#4}}{
          \addplot[rougeTerre, line width=0.15mm, mark=none, opacity=0.8, densely dotted, select coords between index={0}{\nPtDashedMAX}] table[x={x}, y={y}] {#3};
        }{}
      }{}
    \end{axis}
  \end{tikzpicture}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfplotstableread{fibrage_theta1_3_solid.txt}\fibrageSolidCasRationnel
\pgfplotstableread{fibrage_theta1_3_dashed.txt}\fibrageDashedCasRationnel
%
\pgfplotstableread{fibrage_theta1_sqrt2_solid.txt}\fibrageSolidCasAlgebrique
\pgfplotstableread{fibrage_theta1_sqrt2_dashed.txt}\fibrageDashedCasAlgebrique
%
\pgfplotstableread{fibrage_theta1_pi_solid.txt}\fibrageSolidCasTranscendant
\pgfplotstableread{fibrage_theta1_pi_dashed.txt}\fibrageDashedCasTranscendant

% Spectres opérateur de propagation
\pgfplotstableread{eigsP.txt}\eigsP
\pgfplotstableread{numeigs_5percent.txt}\numeigsP

% Solution 1D
\pgfplotstableread{u1DphiQuasi1D.txt}\uPhiQuasiD
\pgfplotstableread{u1Dquasi1D.txt}\uQuasiD
\pgfplotstableread{solLocPertQuasiD.txt}\uLocPertQuasiD
\pgfplotstableread{usolloc.txt}\uLocPertQuasiDsuite


% Erreurs
\pgfplotstableread{erreurs.txt}\erreurs
% \pgfplotstableset{
%   create on use/quasiD_omega1_shift/.style={create col/expr={\thisrow{quasiD_omega1}*exp(-0.1)}},
% }
\pgfplotstableread{polyfits.txt}\polyfits


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Lire un tableau depuis un fichier
\ExplSyntaxOn
\ior_new:N \g_hringriin_file_stream

\NewDocumentCommand{\ReadFile}{mm}
 {
  \hringriin_read_file:nn { #1 } { #2 }
  \cs_new:Npn #1 ##1
   {
    \str_if_eq:nnTF { ##1 } { * }
      { \seq_count:c { g_hringriin_file_ \cs_to_str:N #1 _seq } }
      { \seq_item:cn { g_hringriin_file_ \cs_to_str:N #1 _seq } { ##1 } }
   }
 }

\cs_new_protected:Nn \hringriin_read_file:nn
 {
  \ior_open:Nn \g_hringriin_file_stream { #2 }
  \seq_gclear_new:c { g_hringriin_file_ \cs_to_str:N #1 _seq }
  \ior_map_inline:Nn \g_hringriin_file_stream
   {
    \seq_gput_right:cx
     { g_hringriin_file_ \cs_to_str:N #1 _seq }
     { \tl_trim_spaces:n { ##1 } }
   }
  \ior_close:N \g_hringriin_file_stream
 }

\ExplSyntaxOff

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% \newcommand{\plotmsh}
% Read a file written in the following format
% ------------------------------------------
% number_of_nodes
% index_node,    x_node,    y_node
% number_of_elements
% index_element,   node_1,    node_2,    node_3
% ----------------------------------------------
% Arguments: 1. file name
%            2. nodes color
%            3. elements color
\newcommand{\plotmsh}[3]{
  % \only<1>{
  \ReadFile{\mshelements}{#1}
  % }
  \pgfmathsetmacro\nbnoeuds{\mshelements{1}}
  \pgfmathsetmacro\nbelemts{\mshelements{\nbnoeuds+2}}
  % Draw elements
  \foreach \idI in {1,...,\nbelemts} {
    \pgfmathsetmacro\idsA{{\mshelements{\idI+\nbnoeuds+2}}[1]}
    \pgfmathsetmacro\idsB{{\mshelements{\idI+\nbnoeuds+2}}[2]}
    \pgfmathsetmacro\idsC{{\mshelements{\idI+\nbnoeuds+2}}[3]}
    %
    \draw[#3] ({\mshelements{\idsA+1}}[1], {\mshelements{\idsA+1}}[2])--%
              ({\mshelements{\idsB+1}}[1], {\mshelements{\idsB+1}}[2])--%
              ({\mshelements{\idsC+1}}[1], {\mshelements{\idsC+1}}[2]);
  }
  %
  %
  % Draw nodes
  \foreach \idI in {1,..., \nbnoeuds} {
    \fill[#2] ({\mshelements{\idI+1}}[1], {\mshelements{\idI+1}}[2]) circle[radius=0.5pt];
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Plot curve with linear regression
% #1: file ID
% #2: x label
% #3: y label
% #4: plot options for the curve
% #5: plot options for the regression
% #6: relative position of the triangle
% #7: path for triangle slope
% #8: position of the slope label
% #9: name for slope variable
\newcommand{\plotcurveandregression}[9]{
  \addplot [#4] table [x={#2}, y={#3}] {#1};
  \addplot [#5] table [x={#2}, y={create col/linear regression={y={#3}}}] {#1}
                coordinate [pos=#6] (A) % save two points on the regression
                coordinate [pos={#6 + 0.25}] (B); % line for drawing the slope triangle

  \xdef#9{\pgfplotstableregressiona} % save the slope parameter
     \draw[#5] (A) #7 (B)  % draw the opposite and adjacent sides of the triangle
        % node [pos=0.25, anchor=south] {1} % label the horizontal line
        node [#8] {\pgfmathprintnumber{#9}}; %label the vertical line
}

% Commande \genererFibrage
% 1 : coté du carré
% 2 : abscisse du point de départ de la ligne (relativement au coin inférieur gauche)
% 3 : ordonnée du point de départ de la ligne (relativement au coin inférieur gauche)
% 4 : première composante du vecteur de coupe
% 5 : deuxième composante du vecteur de coupe
% 6 : nombre de composantes de la ligne
% 7 : Longueur de domaine maximale
% 8 : style de tracé
%
% ///////////////////////////////////////////////////////////////////// %
% Attention aux pbs de précision surtout quand on est proche d'un coin. %
% ///////////////////////////////////////////////////////////////////// %
\newcommand{\genererFibrage}[8]{% <-- don't forget this
  \begingroup
    \pgfmathsetmacro\sommetAx{#2}
    \pgfmathsetmacro\sommetAy{#3}
    \pgfmathsetmacro\xextremite{min(#7*#1, (#1 - \sommetAx)/#4, (#1 - \sommetAy)/#5)}
    \pgfmathsetmacro\sommetBx{\sommetAx + \xextremite * #4}
    \pgfmathsetmacro\sommetBy{\sommetAy + \xextremite * #5}
    \pgfmathsetmacro\numIterations{#6-1}
    \pgfmathsetmacro\Lcourante{\xextremite}
    %
    \draw[#8] (\sommetAx, \sommetAy) -- (\sommetBx, \sommetBy);
    %
    % On ne fait la boucle que si la longueur maximale n'est pas encore atteinte
    \pgfmathparse{less(#7*#1, (\Lcourante+0.0001*#1)}
    \ifthenelse{\equal{\pgfmathresult}{0}}{%

      % On ne continue que si le nombre d'itérations est non nul
      \ifdim \numIterations pt > 0pt
      \foreach \idlignes in {1,..., \numIterations} {

      \pgfmathparse{less((#1 - \sommetAx)/#4, (#1 - \sommetAy)/#5)}
      %
      \ifthenelse{\equal{\pgfmathresult}{1}}{%
        \pgfmathsetmacro\nextsommetAx{0}
        \pgfmathsetmacro\nextsommetAy{\sommetBy}
      }{%
        \pgfmathsetmacro\nextsommetAx{\sommetBx}
        \pgfmathsetmacro\nextsommetAy{0}
      }%
      %
      %
      % \ifthenelse{\boolean{#8}}{
      %   \draw[#9] (\sommetBx, \sommetBy) -- (\nextsommetAx, \nextsommetAy);
      % }{}
      \pgfmathsetmacro\nextxextremite{min((#7*#1-\Lcourante), (#1 - \nextsommetAx)/#4, (#1 -\nextsommetAy)/#5)}
      \pgfmathsetmacro\nextsommetBx{\nextsommetAx + \nextxextremite * #4}
      \pgfmathsetmacro\nextsommetBy{\nextsommetAy + \nextxextremite * #5}
      \pgfmathsetmacro\nextLcourante{\Lcourante + \xextremite}
      \draw[#8] (\nextsommetAx, \nextsommetAy) -- (\nextsommetBx, \nextsommetBy);
      %
      %
      % On arrête si la longueur maximale est atteinte
      \pgfmathparse{less(#7*#1, (\nextLcourante+0.0001*#1)}
      \ifthenelse{\equal{\pgfmathresult}{1}}{%
        \breakforeach
      }
      %
      %
      \global\let\sommetAx=\nextsommetAx
      \global\let\sommetAy=\nextsommetAy
      \global\let\sommetBx=\nextsommetBx
      \global\let\sommetBy=\nextsommetBy
      \global\let\xextremite=\nextxextremite
      \global\let\Lcourante=\nextLcourante
      }
      \fi
    }{}

  \endgroup
}

% Pour dessiner fibrages
\newcommand{\tracerFibrage}[4]{
  % #1: première composante du vecteur de coupe
  % #2: deuxième composante du vecteur de coupe
  % #3: nombre de composantes de la ligne
  % #4: boolean; should one show dashed line or not
  \begin{tikzpicture}
    % \pgfmathsetmacro\nPtSolidMAX{3*#1}
    % \pgfmathsetmacro\nPtDashedMAX{3*#1-2}
    \begin{axis}%
      [
        width=0.95\textwidth, height=0.95\textwidth,
        xmin=0, xmax=1, ymin=0, ymax=1,
        xtick={0, 1}, ytick={0, 1},
        enlargelimits=false,
        axis equal,
        unbounded coords=jump
      ]
      \ifthenelse{\boolean{afficherGraphes}}{
        \genererFibrage{0}{0}{1}{0}{0}{#1}{#2}{#3}{line width=0.15mm, bleuDoux};
        % \ifthenelse{\boolean{#4}}{
        %   \addplot[rougeTerre, line width=0.15mm, mark=none, opacity=0.8, densely dotted, select coords between index={0}{\nPtDashedMAX}] table[x={x}, y={y}] {#3};
        % }{}
      }{}
    \end{axis}
  \end{tikzpicture}
}

